Constructing Neural Network-Based Models for Simulating Dynamical Systems

Dynamical systems see widespread use in natural sciences like physics, biology, chemistry, as well as engineering disciplines such as circuit analysis, computational fluid dynamics, and control. For simple systems, the differential equations governing the dynamics can be derived by applying fundamental physical laws. However, for more complex systems, this approach becomes exceedingly difficult. Data-driven modeling is an alternative paradigm that seeks to learn an approximation of the dynamics of a system using observations of the true system. In recent years, there has been an increased interest in data-driven modeling techniques, in particular neural networks have proven to provide an effective framework for solving a wide range of tasks. This paper provides a survey of the different ways to construct models of dynamical systems using neural networks. In addition to the basic overview, we review the related literature and outline the most significant challenges from numerical simulations that this modeling paradigm must overcome. Based on the reviewed literature and identified challenges, we provide a discussion on promising research areas.

==> figures/time_stepper_models/comparison_table.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{|c|c|c|c|}
    \hline
        Name &  Characteristic \\ \hline
        Direct time-stepper & integration scheme   \\ \hline
        ResNet time-stepper & integration scheme  \\ \hline
        Euler time-stepper & integration scheme  \\ \hline
        Neural ODEs &  integration scheme \\ \hline
        Neural State-Space & external input \\ \hline
        Stochastic Time-Stepper & noise \\ \hline
        Recurrent Time-Stepper & noise \\ \hline
        Latent Time-Stepper & noise  \\ \hline
        Hamiltonian Network & energy conservation \\ \hline
        Lagrangian Network &  energy conservation \\ \hline
        Deep Potential Energy & energy conservation \\ \hline
        Graph time-stepper & encode knowledge as graph \\ \hline
        Hiearchical time-stepper & inference speed \\ \hline
        Multi-output time-stepper & inference speed \\ \hline
    \end{tabular}
    \caption{Overview of various types of time-stepper models.}
    \label{tab:ts_comparison}
\end{table}

==> makefile <==
deep_learning_for_dynamical_systems.pdf:
	pdflatex deep_learning_for_dynamical_systems.tex
	bibtex deep_learning_for_dynamical_systems.aux
	pdflatex deep_learning_for_dynamical_systems.tex
	pdflatex deep_learning_for_dynamical_systems.tex

arxiv: deep_learning_for_dynamical_systems.pdf
	zip -FSr arxiv_submission.zip \
		figures \
		sections \
		tables \
		deep_learning_for_dynamical_systems.tex \
		preamble.tex \
		deep_learning_for_dynamical_systems.bib \
		deep_learning_for_dynamical_systems.bbl

csur: deep_learning_for_dynamical_systems.pdf

	mkdir -p csur_submission/pdf
	mkdir -p csur_submission/source
	mkdir -p csur_submission/supplements
	cp deep_learning_for_dynamical_systems.pdf csur_submission/pdf/deep_learning_for_dynamical_systems.pdf
	cp  -r \
		figures \
		sections \
		tables \
		deep_learning_for_dynamical_systems.tex \
		preamble.tex \
		deep_learning_for_dynamical_systems.bib \
		acmart.cls \
		acmart.dtx \
		acmart.ins \
		ACM-Reference-Format.bbx \
		ACM-Reference-Format.bst \
		ACM-Reference-Format.cbx \
		ACM-Reference-Format.dbx \
		csur_submission/source
	cd csur_submission/; zip -FSr ../csur_submission.zip *
	rm -rd csur_submission


==> sections/misc/SurrogateModels.tex <==
\section{Surrogate Models}

Man-made physical systems consist of a large number of subsystems and components, along with their the dynamic interactions. Therefore, these systems can end being highly nonlinear and complex. The simulation of these complex systems can be computationally expensive.

Computational time of larger and complex systems becomes an important factor since the world is shifting toward real-time simulation and cyber physical systems. The resulting simulation system may not be simulated in reasonable time. Therefore, the critical questions ‘How a step can be computed in real-time for monitoring, optimisation, decision making, etc’ arises. Why real time simulation ? 

There are two ways to address this challenge; hardware – modelling approach. Hardware is increasing the computing power or parallel computing. Modelling approach is simplifying the physical model by linearization, convexi., static. An alternative modelling approach to reduce computational time (CPU required time) is through the surrogate models, known as meta models or surface models. 

The use of a surrogate model is a trade-off between accuracy and computational time of the system. What does it mean? Some explanation in here. Surrogate models are built to operate in a larger model in order to expeditiously capture the behaviour of a complex sub-component and therefore provide shorter simulation times of the large model. (Surrogate models are used as substitutes for the complex numerical models.) Learning the behaviour of the model from carrying out experimental measurements or running a limited number of expensive simulations, cases without dependent on the data ‘physical-constraints’. There are multiple tools to create surrogate models, other ML tools. Increasing computational power pave the way to utilise the artificial neural network. (in old times the computational power was not enough to fully benefit of these models cite) Deep neural networks (DNNs), as a class of machine learning techniques, has shown great potential to deal with \textbf{high-dimensional nonlinear uncertainty quantification} problems. 

Structures of the surrogate models is given in Figure X. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/surrogate_structure.png}
    \caption{Structure of Surrogate models}
    \label{fig:Surrogate_structure}
\end{figure}

A system is a simplified representation of reality. A "system" may seem at times an endless series of connected elements with specified boundaries and pre-determined time characteristics. A model is a computer program that describes the mechanics of the considered system, elements of the system. Exercising the surrogate model in conjunction with the simulation is one of the co-simulation techniques

Structure 1: One component is replaced with NN and integrated in a system or a body 
\cite{Ardeh2009} proposed a methodology that replaces the hysteretic nonlinear tire model with a neural network surrogate model that emulates the dynamic response of the actual tire capturing in ground vehicle simulation. Seven simple set of feed-forward NN with one hidden layer including two neurons are used for surrogate modelling. According to the comparison of the CPU times required to run the model in MATLAB and CPU time required by the trained surrogate model, the surrogate model can speed up the simulation significantly. Same methodology is also demonstrated on a full vehicle model with a complex tire element via co-simulation. The results obtained with the surrogate model prove to be accurate and useful for reducing the duration of vehicle simulations.

‘As the number of features or dimensions grows, the amount of data we need to generalize accurately grows exponentially.’ by Charles Lee Isbell. This exponential increase in volume causes high sparsity in the data set, increases storage space and processing time. Limited computing environment hinders the development of the surrogate models. One possible way to avoid this problem is creating the subsystem surrogate models by the decomposition of the model, see \textbf{Structure 2}. Later these two subsystem surrogate models can be simulated in dynamic simulation tool, such in Structure 1 or can be re-integrated into one single surrogate model, such in Structure 3. 

To improve the overall speed of a time-domain simulation of a complex naval system, \cite{ Balchanos2008} built the surrogate model of a small-scale demonstrator consisting of electrical power system, a thermal cooling system and an electro-hydraulic system in recurrent neural network. Decomposition of the system into two physical domains, electrical and thermal cooling, is performed to keep the accuracy required for a reliable surrogate model. These two subsystem surrogate models, they are later integrated into a single surrogate model. The surrogate model was tested against the original monolithic simulation in Simulink. 

Even though, replacing individual components/models with surrogate models in the whole system is promising approach, a large number of components can still lead to time-consuming simulations. Another structure where the surrogate modelling applies is the whole system replacement, see \textbf{Structure 3}. 

In power systems any disturbance creates load unbalances which might cause a cascading series of problems that might eventually cause the loss of the entire grid. To assure the security in the power grids against the possible load unbalances, fast and dynamic simulation are required for effective control actions. With the aim of optimal load-shedding strategies, \cite{ Mitchell2020} has used an architecture of 2 hidden layers neural network to calculate the dynamic frequency response of an island power system where foreseen large amount of wind power production makes the grid vulnerable to the load unbalances. The proposed method replaces whole low-voltage grid including the components connected to the grid with a single surrogate model. Comparison of the results from neural network and a dynamic simulator provides the NN results march with the full dynamic simulations. 

Structure 4: One component is replaced with NN
Structure 4 is generally used to optimise the design of a model. We have eliminated this application due to the scope of this survey. 
\cite{Bender2019} CFD aided by deep Artificial Neural Network (ANN)
\cite{Wu2015} smart water system


Structures of the surrogate models is given in Figure X. 
\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/surrogate_matrix.png}
    \caption{Structure of Surrogate models vs training data}
    \label{fig:Surrogate_structure}
\end{figure}

==> sections/misc/challenges.tex <==
\section{Challenges}

\claudio{Potential challenges: uncertainty and safety \cite{Shafaei2018}}

==> sections/misc/past_input.tex <==
\subsection{Past Inputs}

A rationale for including multiple past states may be that a single observation of the systems state is insufficient to uniquely determine the next state.
For instance, consider if only the angle, and not the velocity, of the ideal pendulum was measured.
Looking at the angle at a single time instance, it is impossible to determine which direction the pendulum is moving.
However, when looking at the angle over multiple time instances, it is possible to estimate its velocity, allowing the network to predict the future state of the system.

Another possible rationale is that feeding past information into the network may simply yield better results in practice.
The idea of a sliding window, is present in many models used across different research disciplines.
For instance, mathematicians define \emph{delay differential equations}, digital signal processing practitioners make use of FIR and IIR filters and in image processing, convolution in 2-d is frequently applied.

\subsubsection{Multi-Input Time-Stepper}

A time-stepper model can be modified to predict future states, based not only upon the current, but also one or more past states.
One way to implement this is to increase the number of inputs passed into the network by the amount of past states included when predicting the next state, as depicted in \cref{fig:time_stepper_multi_in}, which shows the case of a single past state being included.

\begin{figure}
    \centering
    \begin{subfigure}[t]{0.45\textwidth}
    \centering
        \includegraphics[width=\columnwidth]{figures/time_stepper_multi_in.pdf}
        \caption{ }
        \label{fig:time_stepper_multi_in}
	\end{subfigure}
	\begin{subfigure}[t]{.45\textwidth}
    \begin{lstlisting}[mathescape=true]
$x_{win}$ = unfold(x[0:end-1],size=2,stride=1)
$\tilde{x}$ = network($x_{win}$)
loss = MSE(x[2:end],$\tilde x$)
optimizer.step(loss)
\end{lstlisting}
    \caption{Training.}
    \label{lst:ts_multi_in_training}
    \end{subfigure}
	\begin{subfigure}[t]{.45\textwidth}
    \begin{lstlisting}[mathescape=true]
$\tilde x$ = $[x_0,x_1]$
for n in 1...N-1
  $dx$ = network($\tilde x$[n-1:n+1])
  $\tilde{x}$[n+1] = $\tilde x$[n] + h[n]*$dx$
\end{lstlisting}
    \caption{Inference.}
    \label{lst:ts_multi_in_inference}
    \end{subfigure}
    
	\caption{ Multi-input time-stepper}
	\label{fig:ts_multi_input}
\end{figure}

% Another parallel is the recurrent NNs described in \cref{sec:ts_recurrent}.
% Where a multi-input time-stepper explicitly defines the number of past steps included, a recurrent time-stepper learns a set of parameters that determines the contribution of past states to the predicted derivatives.

Training the network is a similar process to other time-stepper, however it requires some processing to form the chunks consisting of the current and appropriate number of past states.
A simplified version of the training algorithm is shown in \cref{lst:ts_multi_in_inference}.
Here \texttt{unfold} refers to a function that extract blocks of a specific size using a sliding window approach.
During inference, the derivative is obtained by feeding chunks consisting of the current and past state(s) into the network, see \cref{lst:ts_node_inference}.

\subsubsection{Recurrent Neural Network} \label{sec:ts_recurrent}

Recurrent Neural Networks~(RNNs) are a class of networks that are commonly used for modeling problems where the output at the current time depends on the previous inputs to the network.
There are several flavors of RNNs such as the \emph{Gated recurrence unit}~(GRU), \emph{Long Short-Term memory}~(LSTM).
Common for all types of RNNs is that they store a representation of their past inputs in a variable that is referred to as the \emph{hidden-state}.
Whenever an input is introduced to the RNN, the hidden state is updated according to a set of update rules that depend on the type of RNN, as well as a set of weights that are tuned during training.

For modeling a dynamical system, an RNN can be used to construct a time-stepper model by setting the hidden dimension to be equal to that of the system and training the RNN such that the hidden state approximates the true state.
Unlike the time-stepper introduced earlier that explicitly utilized the step-size, an RNN does not naturally take into account the step size.
One way to encode this information is to augment the input with the time difference between the current and next sample, which hopefully allows the RNN to account for the potential differences in step size.

\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{figures/time_stepper_models/ts_recurrent_diagram.pdf}
    \caption{Recurrent Neural Network}
    \label{fig:ts_recurrent_diagram}
\end{figure}

In order to use the model for simulation, the hidden state must be initialized to reflect the initial condition.
In this case, the dimension of the hidden state is identical to the dimension of the system, which makes it is possible to initialize the hidden state at $t=0$ by assigning it to the initial state $x_0$.

However, RNNs can also be used in situations where the latent state is not identical to the state of the system.
For instance, the RNN can be used as an encoder that aggregates information over multiple steps, as is the case with the latent time-stepper model described in \cref{sec:ts_latent}.

From a practical standpoint, an RNN can be used to solve the same problem as a time-stepper that uses a numerical solver explicitly.
A difference is that the dependence of step size is introduced by augmenting the input to the RNN and hoping that the network will learn the influence of the step size during the training.
Using an RNN may have the benefit in cases where information from multiple samples are necessary to predict future samples.
For instance, if the observed values are noisy or if a single observation is insufficient to predict the next state of the system.

==> sections/misc/physicalconstraints.tex <==
\section{Physical Constraint Systems}

\begin{itemize}
\item Motivation - why do we need physical constraints in systems?
\begin{itemize}
\item Why? 
\begin{itemize}
\item Consistency
\item Accuracy 
\end{itemize}

\item Which constraints - taxonomy
\begin{itemize}
\item Galilean Invariance
\item Rotation
\item Translation
\item consistency (lake model) 
\end{itemize}
\begin{itemize}
    \item which architecture can handle which constraint
\end{itemize}
\begin{itemize}
    \item Deep tensor neural network
\end{itemize}
\end{itemize}
\end{itemize}


==> sections/misc/scoping.tex <==
\section{Scoping}


\subsection{Modelling vs Simulation}
I suggest we change the scope of the survey to only cover simulation rather than the more broad modelling topic.
This would:
\begin{itemize}
    \item Exclude topics such as soft-sensors and fault-identification
    \item Allow us to focus on properties which are important to a simulation, accuracy, long-term forecasting
    \item More consistent paper that distinguishes itself from others
\end{itemize}

\subsection{Simulation vs Prediction}

In system identification a distinction is made between simulation and prediction.
Simulation refers to the case where model's response to its input and initial state is evaluated.
Prediction is similar, but measurements of its true output are used to correct the model\cite{SimulatePredictIdentified} see fig~\ref{fig:simulation_vs_prediction}

\begin{figure}
    \centering
    \includegraphics{figures/simulation_vs_prediction.png}
    \caption{Simulation vs prediction}
    \label{fig:simulation_vs_prediction}
\end{figure}


\subsection{Multi-step ahead}


\subsection{Physical Systems}

Lets discuss the physical systems part

==> sections/misc/summaries.tex <==
\section{Summaries}

\subsection{Control}



\subsection{Koopman based}

Unlike the their linear counterpart, optimal control non-linear is fundamentally challenging.
Often practitioners want to apply the tried and tested methods known from the linear domain, where theoretical guarantees of convergence exists.
A common approach to this is doing a piece-wise linearization of the systems dynamics.

Another alternative is finding a basis for the state-space that makes the dynamics linear, consider:
$$
x^+ = x^2 
$$

Clearly this can not be expressed as an state-space model:

$$
x^+ = A x
$$

However if we were to augment the input as follows, it would be possible to express it as above:
$$
y = \begin{bmatrix}
x & x^2
\end{bmatrix}
$$

It can be shown that for any non-linear system an finite dimensional mapping of the state exists for which the dynamics are linear.
An active research topic is approximating this function. \cite{korda2018} describes the use of extended-dynamic mode decomposition for this purpose.
\cite{lusch2018} shows how an auto encoder can be applied to approximate the Koopman operator.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/koopman_encoder.png}
    \caption{Approximation of Koopman operator using a Auto Encoder}
    \label{fig:koopman_encoder}
\end{figure}

The nice thing about this approach is that all the tools known from control of linear systems can be applied. Another implication is that concepts known from system identification, such as persistent excitation \cite{boddupalli2019} can be applied to non-linear systems.


\subsubsection{Reinforcement Learning based}
Reinforcement learning has been applied to various tasks within control. 
The idea is that the agent (controller) is trained to perform decisions (control actions) to drive the system to the equilibrium.

For autonomous driving the paper \cite{grigorescu2020} outlines the different steps of this:
\begin{enumerate}
    \item Perception and localisation.
    \item High level path planning, e.g. going from point A to point B.
    \item Behaviour Arbitration, overtaking other cars
    \item Motion controllers
\end{enumerate}

A survey also exists which describes the use of reinforcement learning in the broader context of process control \cite{spielberg2019}

Reinforcement learning requires a model exists such that "what if" scenarios can be evaluated. 
In this sense i don't think this area approach should be considered a use of "DL for modelling". 
Perhaps some knowledge may exists within the fields of creating models for this purpose?

\subsubsection{Soft Sensing}

Soft sensing refers to the use of virtual sensors which approximates physical quantities which are not directly measured. 
A motivation for this is that a quantity may be impractical or expensive to measure.
\cite{shang2014} and \cite{yuan2018} both describe this approach.

The two papers use an example where a physically meaningful quantity is estimated. 
From a practical perspective the network is simply doing regression. 
In this sense soft-sensing and fault identification of non-binary faults are similar.

\subsection{Grey-box Modelling}


==> sections/misc/venues.tex <==
\section{Venues}

\begin{enumerate}
    \item 
\end{enumerate}

==> sections/old_3_simulation.tex <==
\section{Challenges of Neural Network based Simulation} \label{sec:challenges}



% A common critique of NNs is that they are not interpretable and may learn relationships in data that are correlated, but not causal \cite{Karpatne2017}.
% The interpretability of a model can be defined as how easy it for a human to make sense of the results~\cite{Roscher2020}.
% For scientific work these characteristics are highly undesirable since the models will not only be used for prediction, but are also expected to provide an explanation of the cause of the physical phenomenon.

In this section we give an overview of the most common challenges of using Neural Networks as a tool to model and simulate dynamical systems.
First, in~\cref{sec:long_term} we discuss the challenge of obtaining accurate long-term predictions. 
Following this, \cref{sec:robustness} describes the issue of generalization towards unseen initial conditions and inputs.
\cref{sec:missing_data} describes the significance of feeding enough information to the network and describe how networks can be modified to deal with missing or partially observed states.
\Cref{sec:challenge_training} describes the implications of choosing a particular optimization criterion.
\Cref{sec:challenges_speed} gives an overview of techniques for finding a suitable network architecture and determining the optimal hyper-parameters.
%\Cref{sec:optimal_experimental_design} covers techniques designing experiments to obtain data that allows efficient training of the neural network.


\subsection{Accurate Long-term predictions} \label{sec:long_term}

A grand challenge of modeling and simulation is to obtain simulations that remain accurate for predictions spanning long periods of time.
For time-stepping models, the challenge is similar to what is encountered when dealing with conventional ODEs and numerical solvers.
For continuous models, the issue of long term prediction mainly concerns how to make the network work well for any possible input of time.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{figures/model_comparison_CartPendulum.pdf}
	\caption{Prediction of the cart pendulums state produced by the trained networks}
	\label{fig:model_comparison}
\end{figure}

\subsubsection{Error Accumulation in Time-stepping Models} 
\label{sec:error_accumulation_time_stepping}

In numerical simulation, two factors may cause the obtained simulation to deviate from the behavior of the true system: a mismatch between the model defined by the ODEs and the true system; and the discrete sampling performed by the numerical solver.
The first case is attributed to the wrong assumptions made while deriving the ODE, whereas in the second case, the fault lies entirely in the numerical solver.
When modeling the dynamics using a neural networks, no explicit assumptions are made. 
Rather, it is the networks architecture and the incorrect choice of parameters that cause errors.
In the following, we discuss the error introduced by the numerical integration scheme employed by the time-stepping models.
This will help the reader understand how different time stepping models can be compared regarding the error made.

\paragraph{Adaptive Step Size Solvers} \label{sec:adaptive_solvers}

Let us look at the components that make up the forward Euler solver equation, introduced in \cref{eq:fw_euler_solver}.
Intuitively, the larger the step size $h$, the more error the forward Euler solver, can make. \Cref{fig:fw_euler_error}b illustrates this point: by doubling the step size, the error $e(2h)$ became larger than the equivalent error $e(h)$ in \cref{fig:fw_euler_error}a.

\begin{figure}
    \centering
    \includegraphics[width=0.6\textwidth]{figures/fw_euler_error.pdf}
    \caption{Illustration (a) represents the first 4 steps of the forward Euler solver, and (b) the first 2 steps of the same solver with a larger step size. Illustrations (c) and (d) represent the same numerical solver under different step sizes with a slowly changing derivative function.}
    \label{fig:fw_euler_error}
\end{figure}

\claudio{A lot of text went missing here. Please fix this: if you've moved text around, it's your responsibility to make sure things are still tied together. I cannot fix this because I don't know what the original intent of this change was.}
\chris{I did not move this}
To summarize: most numerical solvers are convergent, i.e., the smaller the step size $h$, the smaller the error. To empirically measure the growth rate of the error, see \cref{sec:solver_convergence}.

One can also look at the derivative function $f$, which is another important component of \cref{eq:fw_euler_solver}.
Intuitively, when the magnitude of $f$ is small, the error can be smaller (compare illustrations \cref{fig:fw_euler_error}a and \cref{fig:fw_euler_error}c).

Looking at all illustrations in \cref{fig:fw_euler_error} prompts the question: what if a numerical solver takes smaller step sizes when the magnitude of $f$ is high, and large step sizes when the magnitude is low?
This is precisely what adaptive step size solvers do. These solvers use more sophisticated measures to decide what step size to take, but the principle is the same. We refer 	the reader to \cite{Cellier2006} for an introduction.

The bottom of \cref{fig:ivp_cart_pole_energy} illustrates the step sizes used by the Radau solver, for the simulation of the undamped cart-pendulum system, shown on the top of \cref{fig:ivp_cart_pole_energy}.
As can be seen, the step sizes are smaller when the system is moving faster (when the pendulum is at its lowest point), and larger when the system is moving slowed (when the pendulum is at its highest).

\paragraph{Property Conserving Solvers}

When the pole-cart system illustrated in \cref{fig:system_to_model} has no friction, its energy never changes.

Energy conservation is a property that numerical solvers should mirror:
if a system preserves energy, then the solver should also produce simulations that preserve energy.
To illustrate, the top of \cref{fig:ivp_cart_pole_energy} shows two simulations, produced by two different solvers: the Radau and the Forward Euler (recall \cref{eq:fw_euler_solver}).
It's clear that the Forward Euler fails to mirror energy conservation from the measured energy, which keeps increasing.

\begin{figure}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/ivp_cart_pole_energy}
    \caption{Comparison of Radau and Forward Euler solvers, for undamped (top) and damped (middle) cart-pendulum. At the bottom, we show the step sizes taken by the Radau solver.}
    \label{fig:ivp_cart_pole_energy}
\end{figure}

If the pole-cart system has friction, then it eventually comes to a rest. In other words, it exhibits asymptotic stability.
This too is a property that numerical solvers should reflect (see \cref{sec:solver_convergence} for ways to ensure this).
The middle of \cref{fig:ivp_cart_pole_energy} illustrates the lack of asymptotic stability of the Forward Euler method.
Note how the energy increases over time, instead of decreasing.

\paragraph{Convergence of Numerical Solvers} \label{sec:solver_convergence}

Note that the next term $\tilde{x}_{n+1}$ is approximated from the current approximation $\tilde{x}_n$.
In fact, let $e_n$ denote the error of term $\tilde{x}_n$, so that $\tilde{x}_n = x_n + e_n$, where $x_n$ represents the correct value (see \cref{sec:solver_convergence} for how to compute the current value \claudio{This reference is no longer valid because text was moved around. I don't know where do we explain the analytical solution any more.}).
Then replacing $\tilde{x}_n$ in \cref{eq:fw_euler_solver} makes the accumulation of error clear:
\begin{equation}\label{eq:error_fw}
    \tilde{x}_{n+1} = x_n + e_n + f(x_n + e_n, u(n \cdot h)) \cdot h \\
\end{equation}
The term $f(x_n + e_n, u(n \cdot h))$ can be approximated by a truncated Taylor series expansion:
\begin{equation}
    f(x_n + e_n, u(n \cdot h)) \approx f(x_n, u(n \cdot h)) + \partialder{f(x_n, u(n \cdot h))}{x}e_n \\
\end{equation}
So \cref{eq:error_fw} can be rewritten has:
\begin{aligneq}
    \tilde{x}_{n+1} & \approx
    x_n + e_n + \pargroup{f(x_n, u(n \cdot h)) + \partialder{f(x_n, u(n \cdot h))}{x}e_n} \cdot h \\
    \tilde{x}_{n+1} & \approx
    x_n + f(x_n, u(n \cdot h)) \cdot h  + e_n + \partialder{f(x_n, u(n \cdot h))}{x}e_n  \cdot h .
\end{aligneq}

The resulting expression highlights the fact that $\tilde{x}_{n+1}$ consists of two parts: a Forward Euler step without any previously accumulated error ($x_n + f(x_n, u(n \cdot h)) \cdot h$), and an accumulation of the previously accumulated error, subject to the dynamics of the ODE being approximated $e_n + \partialder{f(x_n, u(n \cdot h))}{x}e_n  \cdot h$.

In short: there are three factors affecting the quality of the approximation $\tilde{x}_{n+1}$:
\begin{itemize}
    \item How good is the numerical method (term $x_n + f(x_n, u(n \cdot h)) \cdot h$ does introduce error);
    \item How difficult is the ODE being approximated (larger term $\partialder{f(x_n, u(n \cdot h))}{x}$ means larger accumulation of errors);
    \item Size of the simulation step (term $h$).
\end{itemize}

Clearly, the simulation step size $h$ plays a fundamental role in the quality of the approximation $\tilde{x}_{n+1}$, as discussed in the next section.
However, some ODEs are very sensitivity to small errors in the state variable (large $\partialder{f(x_n, u(n \cdot h))}{x}$), which means that even small errors (such as floating point precision issues) can caused any long term simulations to be useless.
This is a fundamental challenge in simulating chaotic systems.

\claudio{This paragraph does not make sense. The paragraph on convergence was a few paragraphs above... why is this text here?}
In this section we introduce two performance metrics of a numerical method: its convergence\footnote{The term convergence here refers to the order of the error made by the solver, as the step size is decreased.} and its stability.
We start by introducing a technique to compute the correct solution of a restricted class of ODEs, so that we can later show how to experimentally compute the approximation error of a numerical method, as a function of the step size used.

\paragraph{Analytical Solution}

When the ODE in \cref{eq:ode} has the following form:
\begin{equation}\label{eq:linear_ode}
    \dot{x}(t) = A \cdot x(t),
    \text{with } x(0) \text{ given},
\end{equation}
its solution $x(t)$ is given by
\begin{equation}\label{eq:solution_linear_ode}
    x(t)=e^{At}x_0 \text{, with } e^{At} = I + At + \frac{A^2 t^2}{2!} + \frac{A^3 t^3}{3!} + \ldots,
\end{equation}
where $e^{At}$ is the matrix exponential of $At$ \cite[Section 2.2]{DerekRowell2002}.
This can be verified by taking the derivative of $e^{At}x_0$, and obtaining $A e^{At}x_0 = A x$ (the right hand side of \cref{eq:ode}).

Most software libraries include algorithms to approximate the matrix exponential in \cref{eq:solution_linear_ode}.

The conversion of \cref{eq:solution_linear_ode} to a difference equation can be done by mimicking a numerical method:
\begin{equation}
    x_{n+1} = x(t+h) = e^{A(t+h)}x_0 = e^{Ah}e^{At}x_0 = e^{Ah}x(t) = e^{Ah}x_n.
\end{equation}

This gives us a way to compute a discrete time solution to \cref{eq:ode}, which can be directly compared with an approximate solution of the forward Euler method in \cref{eq:fw_euler_solver}, and therefore used to compute the approximation error.

\paragraph{Approximation Error}

Given an approximation $\tilde{x}(t)$ of the solution $x(t)$ to the IVP introduced in \cref{eq:linear_ode}, we define the approximation error of an approximation computed with step size $h$ as $e_h (t) = x(t) - \tilde{x}(t)$, and the maximum error up to a finite $T>0$ as $e_{\mathop{max} T}(h)=\max_{i \in \set{0, \ldots, T/h}} \norm{e_h(ih)}$.
%When we want to highlight the maximum error as a function of $h$, we denote it as $e_{\mathop{max} T}(h)$.

We can experimentally plot the error $e_{\mathop{max} T}(h)$ of a numerical method applied to an IVP as a function of the step size $h$ as follows. Pick a finite simulation time $T>0$; and compute the maximum error $e_{\mathop{max} T}(h)$ of the analytical and numerical solutions up to $T$ for different step sizes.
\Cref{fig:convergence_euler_vs_midpoint}, adapted from \cite{Gomes2018c}, shows this plot for two numerical methods.

The resulting $e_{\mathop{max} T}(h)$ can be used to get the empirical \emph{order} of the numerical method.
Roughly, for sufficiently small $h$, if $e_{\mathop{max} T}(h) < c \abs{g(h)}$ for a given function $g(h)$ and positive constant $c$, then we say
that $e_{\mathop{max} T}(h)$ is in the order of $g(h)$, or in other words, $e_{\mathop{max} T}(h) = \bigO{g(h)}$.
The constant $c$ that approximates the error depends on the IVP being solved, but the order is a property of the numerical method \cite[Section I.7 and II.1]{Wanner1991}.

\begin{figure}[tbh]
    \begin{center}
        \includegraphics[width=0.7\textwidth]{figures/convergence_euler_vs_midpoint}
        \caption{Empirical approximation order of the explicit Euler and the Midpoint methods. Taken from \cite{Gomes2018c}.}
        \label{fig:convergence_euler_vs_midpoint}
    \end{center}
\end{figure}

\Cref{fig:convergence_euler_vs_midpoint} illustrates well the simulation speed vs accuracy trade-off: smaller step size leads to better accuracy, but means the simulation takes more time as there are many more equation evaluates for a finite time interval.

A similar analysis can be done to NNs that accept a step size as input: does it truly exhibit the convergence property?
We show empirically in \claudio{Christian, please add our own plot here, and update this paragraph} that this is not the case.
As the figure illustrates, when we decrease the step size of a NN trained with a fixed step size, the error does not become necessarily smaller.
Compare this with \cref{fig:convergence_euler_vs_midpoint}.

In the SoTA, this is the question posed and answered in \cite{Ott2020}.
The authors demonstrate that Neural ODEs are not necessarily convergent, but they can be made convergent through training.
They propose an extended method for training the network to make it invariant to step-size.


\paragraph{Stability}

\jan{Write about stability here}

We now introduce the concept of stability of an ODE, and derive the conditions under which the numerical methods introduced in preserve this property.
We take the simplest definitions, and refer the reader to more details in \cite[Section 2.3]{Stuart1998}.
The derivation of the conditions for stability of vector ODE's is taken from \cite[Section I.12]{Wanner1991} and \cite{MIT2009}.
For the stability of adaptive numerical methods (e.g., ones that change the step size over time), we refer the reader to \cite{Gomes2017,Gomes2018b,Gomes2018a}.

We say that the ODE in \cref{eq:ode} is \emph{asymptotically stable} when all its solutions tend to zero as time passes, regardless of the initial value. The cart-pendulum ODEs an example of an asymptotically stable system since both cart and pendulum will eventually come to a halt due to friction.
Formally, $\lim_{t \to \infty} \norm{x(t)} = 0$ for all $x(t)$ satisfying \cref{eq:ode}.

A scalar ODE in the form of
\begin{equation}\label{eq:scalar_linear_ode}
    \dot{x} = ax
\end{equation}
is asymptotically stable if $a<0$.
The analogous condition for vector ODEs of the form of \cref{eq:linear_ode}
is that the real part of all eigenvalues of $A(\theta)$ is strictly negative \cite[Section I.12]{Wanner1991}:
\begin{equation}
    \forall \lambda_{j} \in Re(\lambda{(A)}),\ Re(\lambda_{j}) < 0.
\end{equation}
These conditions can be checked automatically.

To see why a numerical method may fail to preserve the asymptotic stability of a system of differential equations, consider a scalar ODE in the form of \cref{eq:scalar_linear_ode}, and apply the explicit Euler method (\cref{eq:fw_euler_solver}) to get
$x(t+h) \approx x(t) + a h x(t) = (1 + a h) x(t) = (1 + a h)^{n} x(0)$, where $n=t/h$.
For any $x(0)$, the term $(1 + a h)^{n} x(0) \to 0$ as $n \to \infty$ if $\abs{1 + a h} < 1$.
Note that the larger $\abs{a}$ is, the smaller the step size has to be, in order for the method to be numerically stable.

The vector version of the above derivation is analogous.
Consider a vector ODE in the form of \cref{eq:linear_ode}, and apply the forward Euler method (\cref{eq:fw_euler_solver}) to get
$x(t+h) \approx (I + A h)^{n} x(0)$, where $n=t/h$.
For any $x(0)$, the term $(I + A h)^{n} x(0) \to 0$ as $n \to \infty$ if $\rho(I + A h) < 1$ \cite{Strang1993}, where $\rho(\cdot)$ denotes the maximum absolute eigenvalue of $\cdot$, also called the spectral radius of $\cdot$.

The procedure to decide the \emph{numerical stability} is summarized as follows.
Apply the equation representing the numerical approximation to a differential equation of the form of \cref{eq:linear_ode}, and obtain an equation with the form
\begin{equation}\label{eq:dts}
    x(t+h) \approx \tilde{A} x(t)
\end{equation}
where $\tilde{A}$ is a constant matrix.
Then check whether $\rho(\tilde{A}) < 1$.

For ODEs that are non-linear in the state, this algorithm can be applied to a linearization of the ODE around an equilibrium point, or, preferably, more general methods can be used to prove stability, such as the use of Lyapunov function to show, by induction, that the solution remains bounded (see, e.g., \cite{Fridman2014} and references thereof).
See also \cite{Gomes2018d} for examples of stability analysis to different numerical methods.


\subsubsection{Extrapolation in Time Of Continuous Model}
Unlike a time-stepping model a continuous models does not suffer from the accumulation of error due to integration. 
However it has its own limitations in regards to producing accurate long term prediction.
Specifically, the network must be trained with samples that are sufficiently dense in both temporal coordinates.
For short prediction spanning from 0 to 1 seconds this may not be an issue. 
However, if the model is asked to predict the interval of 0 to 10 seconds, without retraining it with samples corresponding to the new time interval, it will likely perform poorly.
\claudio{Can we find some more evidence for this, or some explanation? It feels like a claim we ought to justify.}
\chris{Perhaps we should just claim that there is no reason to assume that the network will work for points which it has not been trained for}

\subsection{Generalization Towards Unseen Initial Conditions and Inputs} \label{sec:robustness}

A common phenomenon encountered during the training of NNs is \emph{overfitting}; the optimizer may find a set of parameters that works very well on the training data, but poorly on other data.
For NNs trained to do simulation this consequence is that the model is only guaranteed to work for the specific combinations of initial states and inputs used to train the network. 

One way to mitigate this issue is to obtain training data that is representative of more dense set of initial conditions and inputs.
However, obtaining more data is not always feasible, especially if it has to be measured from the physical system through experiments.
This issue is further aggravated when dealing with a systems that have high dimensional state-space.

\subsubsection{General Regularization Techniques}
An alternative approach is to use \emph{regularization} that penalizes choices of network parameters that are characteristic of the network overfitting.
Two common choices are L2 and L1-regularization \cite[page 226]{Goodfellow2016} which are realized as additional terms in the loss function used during training of the network:
\begin{equation}\label{eq:generic_cost_function}
	\mathcal{L} = 	\underbrace{\frac{1}{N}\sum_{i=0}^{N} ||{x_i-\tilde{x}_i}||_2}_\text{prediction error} + 
	\underbrace{\alpha \sum_{j}^{M}||w_j||_1}_\text{L1-norm} + 
	\underbrace{\beta \sum_{j}^{M}||w_j||_2}_\text{L2-norm}.
\end{equation}
\claudio{What are the symbols of this equation? $N,M$. Please explain what they are, or remind the reader of what they are.}

The L1 norm favors weights where the sum of coefficients~(taking the absolute value) are small
Contrary to this, the L2 regularization favors weights where each coefficient is small, leading to dense solutions.

Another popular regularization technique is \emph{dropout}, implemented by zeroing the contribution of weights during training for a randomly selected fraction of neurons during training.
Some intuition for why this works is that networks that rely heavily on few neurons for prediction are very susceptible to those neurons dropped.
\claudio{citations for dropout?}


\subsubsection{Physics Informed Regularization}

As discussed in \cref{sec:long_term}, sometimes constraints or invariants of the system are known.
These can be easily incorporated as extra regularization terms in \cref{eq:generic_cost_function}.

\jan{Write about physics-informed NN here}

\claudio{I think this is already written in \cref{sec:continuous_model}. Why are we repeating the same content here?}

\subsubsection{Choosing the Right Experiments} \label{sec:optimal_experimental_design}

\claudio{TODO: After we have a consistent draft, check whether this section should be linked to our cart pendulum system. We can simply show what happens if a cart pendulum NN is trained with initial conditions that are scaling of themselves, vs it being trained with initial conditions that are randomly sampled.}

In the following, we highlight the problem of determining whether a training set is good, and/or how to generate a good training set.
Then we give an overview of the different methods to tackle this challenge in SoTA, focusing on those that have been or can be applied to dynamical systems prediction.
We can single out two motivations for the importance of having the right experiments: reducing costs in generating labeled training data \cite{Settles2009a}; and training networks with less bias.

Different sets of training data will result in different models.
The challenge can be broadly posed as follows: what is the optimal training data set $X$, for which a given network $N$, after training on $X$, will perform optimally on its tasks?

In the SoTA, this problem is related to optimal experimental design \cite{Siciliano2008}, active learning \cite{Settles2009a}, and generation of persistently exciting inputs \cite{Green1986}:
optimal experimental design works by measuring the effect of adding or exchanging data points to the training outcome;
the key idea behind active learning is that a machine learning algorithm can achieve greater accuracy with fewer labelled training instances if it is allowed to choose the data from which it learns; and persistency of excitation studies the shape the inputs that ensure maximum identifiability of the system.
This problem is also important for model reduction using auto encoders \cite{Vincent2010}, where data produced by a more complex model is used to train a simpler model. 
The better the data is, the better the reduced model will perform.

In the SOTA, we can distinguish approaches based on whether they use information about some kind of model of the system, or not.
Most of the DL approaches fall into the later category, since the neural network does not encode any structure that correlates to the structure of the system.
The approaches that are based on the existence of a model have a major advantage over the approaches that do not do so, because the models represent physically-based approximations of the structure of the system, and they can be used to guide the generation of training data.
DL approaches on the other hand do not have this information.

Model-based approaches can be subdivided into linear and non-linear models (the linearity being with respect to the parameters of the model, as opposed to the linear SSMs, in ).
More details about optimal design of experiments for linear models can be found in \cite{Pukelsheim2006} and for non-linear models can be found in \cite{Boddupalli2019}, and for both in \cite{Isermann2010} with a focus on dynamical systems.

We can also distinguish between open and closed loop approaches. 
Open loop approaches try to generate good training data without trying to train the network, and closed loop approaches train the network and adjust the data accordingly.
Open loop approaches are based on maximizing auto correlation of the data.
As an example of the open loop approaches, we have the maximization of cross correlation functions on the inputs and outputs of the system; or the minimization of the trace of an expression based on Fisher's information matrix \cite{Shoham2020}.
As an example of closed loop approaches, we have the minimax approach described in \cite{Welsh2006} (from \cite[Sect 23.1]{Isermann2010}), and more in \cite{Settles2009a,Shoham2020,Shao2019,Sato2013}.

\begin{figure}
	\centering
	\includegraphics[width=.7\textwidth]{figures/error_distribution_CartPendulum.pdf}
	\caption{Distribution of errors committed by different models for trajectories in training and validation set. The width denotes the probability and the 1-axis the error. \claudio{What is this figure doing here? It is never referenced.}}
	\label{fig:prediction_err_distribution}
\end{figure}

% \subsection{Dealing with Noisy and Partial Observations} \label{sec:missing_data} % moved to 4_time_stepper_models

% \claudio{This whole sub-section needs a rewrite.}

% One issue than can arise when modeling the dynamics of a system is that the observed states used to train the model may be corrupted by noise as in 
% $y_k = x_k + \epsilon$, 
% where $\epsilon$ is a random distribution.
% Additionally, there may be cases where measurements of the entire state-space are unavailable and instead only a \emph{partial} description is available \cref{eq:state_partial}.
% \begin{equation} \label{eq:state_partial}
%     y_k = M x_k
% \end{equation}

% \claudio{Do we need the above two equations? It seems they don't add much to the text that comes next.}

% Hidden physics networks specifically deal with these issues \cref{sec:hidden_physics}.
% \claudio{What is this reference for?}
% \claudio{In the rest of this paragraph, are we still talking about hidden physics networks?}
% During inference, partially observed state is an issue for time-stepping models since the network is lacking the sufficient information to predict the next state.
% For example consider if only the position of the cart and the angle of the pendulum was known, then there would be no way of knowing the velocity of the pendulum.
% Likewise any perturbations of the initial conditions will lead to a different trajectory since the network the model will treat this as a fundamentally different experiment.

% One way to deal with this is to provide both the current and a number of past states to the network as described in \cref{fig:time_stepper_multi_in}.
% Alternatively, the model can be made to remember past inputs as described in \cref{sec:rnns}.

% The separation of observed and hidden state is useful when a single input does not contain enough information to predict the next state or is when it is corrupted by noise.
% The authors of \cite{Chen2019} proposed a \emph{latent-ode} model that uses an RNN to encode several noisy observations to a single point in a latent space.

% The concept of a simulation model can be thought of as an generalization of an IVP: 
% \begin{equation*}
% 	\underbrace{[\hat{x}_0,\hat{x}_1,...,\hat{x}_N]}_\text{predicted states} = 
% 	M(
% 	\underbrace{[y_0,y_1,...,y_k]}_\text{observed states},
% 	\underbrace{[u_0,u_1,...,u_N]}_\text{inputs},
% 	\underbrace{[t_0,t_1,...,t_N]}_\text{timestamps}
% 	),
% \end{equation*}
% \claudio{are we set on the name ``simulation model''? I would more likely call it ``sensor fusion model'' or something along those lines. And how is it a generalization of the IVP? That's like saying a Kalman filter is the same as a simulator. The two are very different.}
% the notable differences being that a distinction is made between observed and true state, $y_i$ and $x_i$.
% This distinction is made to accommodate cases where the true state at $t=0$ is only partially known or corrupted by noise.

% Related to this issue is the fact that a simulation model may take multiple samples of the observed state compared to the single sample required for solving an IVP.
% \claudio{This paragraph looks like an afterthought}

% One drawback of this model is that the hidden state takes several samples to converge on a value that results in a correct prediction.

% \thomas{Blend in following text with the rest.}
% For applications such as MPC, the true state of the system at a given time time may not be known, making it challenging to predict how the system will behave in the future.
% The uncertainty of the systems state can be caused by sensor noise or simply the fact that some no sensors exist that may measure the physical quantity directly. In such cases the state must be estimated indirectly by examining how the system behaves in some time window.

% A common approach to this to this problem is using an encoder network to obtain a representation in a latent space by feeding in several measurements of the observed state. An example of this for the cart pendulum would be if we used a camera to observe the position of the pendulum and the cart, but not their velocities. Looking at a single observation there is no way of determining which way the system is moving or at which rate.
% However, looking at multiple samples it is possible to determine which way and at what speed the system is moving. \chris{Add example which shows a good and a bad network structure for this}

% \claudio{We don't need to create subsubsections if we don't have significant content for them.}

% \subsubsection{Feeding multiple States into Network}
% Another approach is to feed multiple sample to the network at each step \cref{fig:time_stepper_multi_in}.

% \begin{figure}
% 	\begin{subfigure}[t]{0.6\textwidth}
%     \centering
%         \includegraphics[width=\columnwidth]{figures/time_stepper_multi_in.pdf}
%         \caption{ }
%         \label{fig:time_stepper_multi_in}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{0.6\columnwidth}
% 		\centering
% 		\includegraphics[width=\textwidth]{figures/time_stepper_recurrent.pdf}
% 		\caption{ }
% 		\label{fig:time_stepper_hidden_state}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{0.6\textwidth}
% 		\centering
% 		\includegraphics[width=\columnwidth]{figures/time_stepper_latent_ode.pdf}
% 		\caption{ }
% 		\label{fig:time_stepper_latent_ode}
% 	\end{subfigure}
% 	\caption{Strategies for dealing with partial and noisy state in time-stepping models}
% 	\label{fig:dealing_with_partial}
% \end{figure}




% \subsubsection{Encoding Past in Hidden State} \label{sec:rnns}

% In Recurrent Neural Networks~(RNNs) the prediction of $x_{k+1}$ does not depend on $x_k$ alone but also on samples from the past. RNNs use what is called a hidden state to retain information about past inputs. The hidden state of the network and the state of the system are two entirely different things and should not be confused; while the hidden state is influenced by previous system states it usually has a different dimensionality and lacks any obvious connection to the system state. The values in the hidden state are typically used in conjunction with the input to the network in a fully connected layer that maps them to a prediction of the next system state. Updates to the hidden state are governed by the \emph{gating mechanism}; it balances the influence of the current input to the network and the influence of current hidden state on the next hidden state.

% \subsubsection{Encoding and Solving In Latent Space}

% One way to deal with a noisy or partial estimate of the initial state is to use an auto-encoder \cref{fig:time_stepper_latent_ode}, referred to by \cite{Chen2019} as \emph{latent-ode}.
% Specifically a number of observed states $[y_k,y_{k-1},...,y_0]$ samples are used to obtain a single initial state, $\tilde{z}_0$ which represents all the relevant information aggregated from the observed states.
% $\tilde{z}_0$ is used as the initial condition to solve the ODE in the latent space, yielding $[\tilde{z}_0, \tilde{z}_1,... ,\tilde{z}_n]$.
% Finally, the solution of in the latent space is mapped back to the initial state-space by a network $G$, to obtain the solution $[\tilde{x}_0,\tilde{x}_1, ..., \tilde{x}_n]$.

% \subsection{Difficulty Optimizing Parameters of Network} \label{sec:challenge_training} % moved to 4_time_stepper_models and 3_continuous_time_models

% A fundamental challenge of data-driven modeling of non-linear systems using NNs is that the loss function is highly non-convex, eliminating any guarantee that the gradient-descent based optimizer will arrive at a global minimum.
% In other words, even if the network is sufficiently rich to the model the system, there is no guarantee that an optimizer will converge on a set of parameters that results in a perfect fit with the system.

% Fortunately, in many situations we are satisfied with a non-zero error, provided that it is sufficiently small for the particular use of the prediction.
% Related to this is how to quickly and reliably train the network to reach a acceptable error.
% Finding effective ways to optimize neural networks is an diverse and active research area.
% Some of this research is focused on developing techniques such as robust optimization algorithms \cite{Kingma2017} and batch normalization \cite{Ioffe2015, Santurkar2019}, that can be applied effectively to a broad class of problems.

% It should be emphasized that the optimization process is also heavily influenced by the networks architecture. 
% For example, very deep networks can take a long time train because gradients of the output with respect to the weights of the earlier layers tend to vanish \cite[page 286]{Goodfellow2016}.
% Multiple strategies have been proposed for mitigating this issue, some targeting the initialization of weights \cite{Glorot2010}, the structure of the network such as \emph{skip-connections} proposed by~\cite{He2015}, or choosing a different activation function \cite{Talathi2016}.

% More specific to the topic of this paper are the techniques that exploit the fact that the system should behave like a dynamical system.
% For example an loss function can be chosen that is easier to optimize than the naive approach as described in \cref{sec:training_time_stepping}.

% \subsubsection{Optimization Criterion For Time-Stepping Model} \label{sec:training_time_stepping}
% Neural Networks can be trained to minimize different quantities, some of which result in an better optimization landscape than others \cref{fig:computation_graph_step_sim}.
% One can view the right hand side of \cref{fig:computation_graph_step_sim} as a very deep network (layers equal to number of steps) and the left hand side as a single layer.
% \claudio{Text to be finished.}


% \begin{figure}
%     \centering
%     \begin{subfigure}[t]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/prediction_minimize_step_vs_sim.pdf}
%         \caption{Prediction obtained from the trained model.}
%     \end{subfigure}
%     \begin{subfigure}[t]{0.48\textwidth}
%         \centering
%         \includegraphics[width=\columnwidth]{figures/computation_graph_step_sim.pdf}
%         \caption{Computation graph resulting from minimizing single-step error and simulation error during training. $f$ denotes the function implemented by the forward pass of the NN.}
%         \label{fig:computation_graph_step_sim}
%     \end{subfigure}
%     \caption{Comparison of different optimization criterion for the same model.}
% \end{figure}

% \chris{
% \begin{itemize}
% 	\item lift state-space to higher dimension to ease optimization \cite{Dupont2019}
% 	\item ODEs are not unconditionally as assumed by reversible \cite{Gholami2019}
% 	\item One way to make time-stepping networks converge faster is to favor simpler ODEs rather than complex wiggly ones \cite{Finlay2020}.
% \end{itemize}
% }

% \subsubsection{Training PINNs}
% Training PINNs effectively using gradient descent based methods requires careful tuning of the learning rate. 
% Specifically it has been observed that the boundary conditions and the physics regularization terms may converge at different rates leading.
% In some cases this manifests itself as a large misfit specifically at the boundary points.
% The authors of \cite{Wang2020a, Wang2020} propose a strategy for weighing the individual terms of the loss function may lead to consistent minimization of all terms, resulting in a lower total error. 

% \claudio{I stress that the content in this subsection is very good, and does not need to be structured into subsubsections. Each subsubsection is basically a paragraph. See \cref{sec:optimal_experimental_design} for an example of how to structure the subsection.}

% \subsection{Decreasing Inference Times} \label{sec:challenges_speed} % moved to 4_time_stepper
% For some applications the NN-based model must have a sufficiently low inference time to allow for real-time predictions.
% This is especially relevant in cases where the NN-based model is used as a surrogate for a slower model, derived through other means.

% Continuous models can be easily parallelized since the output of the model at a given time is independent of the output at previous times, as seen in \cref{fig:continuous_model}.
% This means that the solution can be evaluated at multiple times in constant time, $\mathcal{O}(1)$, provided sufficiently capable hardware.
% Contrary to this, the prediction of a time-stepping network depends on the past predictions resulting in an inference time that scales linearly with the number of steps, $\mathcal{O}(n)$.
% It should be noted that the time-stepper models are capable of simulating multiple trajectories corresponding to multiple initial conditions in parallel, which may be useful for some applications.

% There are two ways to reduce the total amount of time: 1) reduce the number steps, 2) reduce the time each step takes.
% One way of that of reducing the number of steps necessary is to predict multiple future states of the system for each invocation of the system using \emph{multi-step} prediction, as seen in \cref{fig:time_stepper_multi_out}. 
% Another, way is to use several networks that performs predictions at different time-scales and then aggregate the results to form the final prediction as shown in \cref{fig:time_stepper_hierarchical}.

% \begin{figure}
% 	\begin{subfigure}[t]{0.45\textwidth}
%     \centering
%         \includegraphics[width=\columnwidth]{figures/time_stepper_multi_out.pdf}
%         \caption{ }
%         \label{fig:time_stepper_multi_out}
% 	\end{subfigure}
% 	\begin{subfigure}[t]{0.45\textwidth}
% 		\centering
% 		\includegraphics[width=\columnwidth]{figures/time_stepper_hierarchical.png}
% 		\caption{ \chris{placeholder \cite{Lu2018}}}
% 		\label{fig:time_stepper_hierarchical}
% 	\end{subfigure}
% 	\caption{Ways to reduce number of function evaluations of time-stepping model}
% 	\label{fig:time_stepper_reducing_evaluations}
% \end{figure}

% \subsubsection{Multi-step Models} \label{sec:time_stepper_multi_out}
% One approach to obtain a prediction of several steps is to train a fully-connected NN to obtain all of these at once based on a single initial state, as depicted in~\cref{fig:time_stepper_multi_out}.

% \subsubsection{Hierarchical Time-Stepper} \label{sec:hierarchical_models}
% \emph{Hierarchical Time-Stepper}~\cite{Liu2020} reduce the number of function evaluations using a collection of networks trained to take different step sizes \cref{fig:time_stepper_hierarchical}.

\subsubsection{merge this stuff into above}
% Motivation for fast models
\claudio{Add citation to each kind of analysis}
Models are used as basis for sensitivity analysis, optimization, uncertainty quantification, real-time monitoring, fault diagnoses, \claudio{Anything else?}.
These often require numerous simulation runs, or that each run can progress in the simulated time as fast as the wall clock time.
Obtaining computationally efficient models is therefore crucial.

% Distinction
We distinguish two situations: 
\begin{compactdesc}
\item[Data Driven] the user has data and wants to build a fast model, and 
\item[Model Reduction] the user already has a model, and wants to make a faster model.
\end{compactdesc}
% Comparison
The two approaches share some similarities. For example, data produced by a slow model can be used to produce a faster model, using a data driven approach.
However, the model reduction process can make use of the special structure of the model to more efficiently produce a faster model.
Moreover, data driven approaches are dependent on the quality of the data, a challenge we revisit in \cref{sec:optimal_experimental_design}.

% Data driven outside context of DL.
Data-driven approaches generate approximations of the high-fidelity model by using interpolation or regression of simulation data from the input/output relationships.
Outside the context of DL, there are popular approaches such as polynomial regression, radial basis functions, kriging, neural networks, support vector regression, Gaussian process regressions, fuzzy systems, as summarized in \cite{Forrester2009}.
For a recent and general discussion on data driven approaches, we refer the reader to \cite{Koziel2020} and \cite{Mohammed2018}.

\paragraph{Broader Surveys on Model Reduction}

% Surveys on model Reduction outside context of DL.
Model reduction approaches typically make use the equations representing a dynamical system with a large number of state variables, to produce a model of a dynamical system with a lower number of state variables, while approximating the input/output behavior of the original model.
We can distinguish these approaches by the assumptions they make about the structure of the original model.
For a discussion on model reduction of linear models, we refer the reader to \cite{Antoulas2000}, for differential algebraic equations, we refer to \cite{Benner2017}, and for models that depend on a set of parameters, we refer the reader to surveys on model reduction to parametric models \cite{Benner2015,Swischuk2019}.

\paragraph{DL Based Surrogate Modeling}

The network architecture affects the performance of the NNs.
One of the often cited benefits of NNs is that they can parallelize processing of data on specialized hardware such as GPUs \claudio{Citations?}. 
While this is true it is important to recognize what type of parallelism the use of NNs provides.
Similar to conventional multiprocessing, only tasks that are independent in the sense that they do not rely on the result of the other can be parallelized. 
An example of a model that can efficiently use a GPU is the model seen in \cref {fig:time_stepper_direct}, which takes a single sample and produces N samples in one iteration.
Different from this is the model in \cref{fig:time_stepper_euler}, where each new iteration of the network relies on the previous one.
The difference in performance grows linearly with the number of samples predicted into the future. 
A compromise can be made by predicting several steps into the future for exact input, as done in \cite{Forgione2020}.
\chris{Show results where chunked prediction is made}

The traditional DL approaches require large amounts of training data \cite{Hartmann2018}, but require less domain knowledge, and both training and evaluation can be done in GPUs, boosting their performance \cite{Andersson2019}.
DL architectures such as the deep auto encoders have been shown to be more flexible than traditional Proper Orthogonal Decomposition (POD) approaches.
Some contributions leverage the link between POD and auto encoders \cite{Baldi1989} to train neural networks \cite{San2018,San2019,Hartman2017}.
This allows for an implicit representation of the time evolution of the temporal POD modes without performing a Galerkin projection, thereby improving the performance.
These approaches, just as with POD approaches, focus on finding the system dynamics (rate of change), as opposed to predicting the system's subsequent state evolution, and therefore need a numerical solver and iterative computation to perform prediction of system behavior.

Approaches that focus on predicting the system's behavior bypass the numerical solver and therefore have a higher performance, since they can be evaluated in parallel.
\claudio{Refer to the different NN architectures described in the previous sections, instead of the following sentence:}
Long Short-Term Memory \cite{Mohan2018}, Residual Networks \cite{Chang2018}, and the incorporation of numerical solvers as regularization \cite{Raissi2018a}, have been shown to require less training data to accurately predict system evolution.
Recent developments have focused on incorporating domain knowledge into the training process, and architecture of the network \cite{Rueden2020a}.
Within the manufacturing domain, a data-driven method exploiting a neural network to approximate the state space model for mould cooling in injection molding process was proposed in \cite{Everett2017}. Recent advances in applying DL to the fluid mechanics domain are summarized in \cite{Brunton2020}.

The task of applying model reduction to a DL is also known as: as network distillation, hyper-parameter tuning, model selection, \claudio{What else?}.
Intuitively, as in done in traditional system identification, \cite[23.3.2]{Isermann2010}, and described in \cite[1.3 Parameters]{Pronzato2013}, one possible approach is to plot the behavior of the cost function of the optimal parameters found, as a function of the network architecture. In such a plot, the best number of network parameters is the smallest number for which the cost does change significantly.
If white noise is present in the data, then we can increase the order of the network until we can observe that the residuals (errors of the optimal parameter selection for the network) are close to white noise (whiteness can be tested using auto-correlation.)

\alexandros{If we are going to draw connections to new concepts from the ML side in the sections (wherever possible), we can also state here that when the problem is seen from the neural network's topology/hyper-parameters/parameters point of view, recent Neural Architecture Search methodologies (including very time-consuming ones following meta-learning, and progressive learning methods) can be used}

\claudio{The structure of the network can be fined tuned using sensitivity based methods. For instance, \cite{Cheng2019}.}

\claudio{As a possible discussion point, maybe we can claim that interesting research might be carried out in training or analyzing NNs that can be broken up into small pieces, so that their simulation can be carried out in parallel, with occasional synchronization. Just like what is done in the world of parallel and distributed co-simulation \cite{Gomes2018}.}

\claudio{Research questions for co-authors, whose answers may lead to discussion points in this section}
\begin{compactitem}
\item Are there contributions on DL based model reduction for parametric models?
\item Are there contributions on DL based model reduction of Differential Algebraic Equations.
\item Which of the papers you've read is doing any kind of systematic architecture optimization?
\end{compactitem}

==> sections/old_4_advanced_topics.tex <==
\section{Advanced Topics} \label{sec:advanced_topics}

\chris{The contents of this section are either merged into \cref{sec:challenges} or cut}

\subsection{DAEs and PDEs}

\begin{definition}
    \textbf{A system of Differential Algebraic Equations (DAE)}:
    in explicit form expands ODE~\cref{eq:ode} by including a set of algebraic equations $\mathbf{g}$:
    \begin{equation}
        \label{eq:dae}
        0        = \mathbf{g}(\mathbf{x}(t)^{n-1}, \ldots, \mathbf{x}(t)', \mathbf{x}(t), \mathbf{u}(t))
    \end{equation}
\end{definition}

\begin{definition}
    \textbf{A system of Partial Differential Equations (PDEs)}:
    is given in implicit form as
    \begin{equation}
        \label{eq:pde}
        0 = \mathbf{f}({x}_1, \ldots, {x}_n, {y}_{{x}_1}, \ldots, {y}_{{x}_n})
    \end{equation}
    Here the standard notation is slightly different and variables ${x}_i$ may represent spatio-temporal dimensions of the problem, while  ${y}$ represents some physical variable of interest, e.g. heat or concentration.
    The notation ${y}_{{x}_1}$ represents partial derivatives using subscripts:
    \begin{equation}
        {y}_{x_1} = \frac{\partial y}{\partial x_1}, \  {y}_{x_1,x_1} = \frac{\partial^2 y}{\partial x_1^2}, \  {y}_{x_1,x_2} = \frac{\partial^2 y}{\partial x_1 \partial x_2}
    \end{equation}
    Where in physics, the second-order differential operator
    is often called a Laplace operator denoted as:
    \begin{equation}
        \Delta {f} = \sum_i^n \frac{\partial^2 {f}}{\partial x_i ^2}
    \end{equation}
\end{definition}



\subsection{Model Reduction and Surrogate Modelling}

\jan{I dont think we should be covering model reduction into such extent as laid down right now. Lets focus on simulations as stated by the title.}

\claudio{What's the difference between the above two?}

\chris{How can we relate the use of NNs to model reduction? I think showing how a NN-based model of the pendulum can be refined would be a good way to show this. For example a model with 10000 parameters could be reduced to one with a 100}
\begin{itemize}
    \item How can NNs be used to accelerate simulation
    \item Give an example, autoencoder, pole-cart
    \item Mention parallel to PCA
\end{itemize}

\subsection{Surrogate Modelling}


\subsubsection{Surrogate Model Selection}

(Since there is no clear taxonomy of the surrogate modelling categories in the literature,) in this paper, surrogate modelling are divided into three categories based on mathematical applications; Data-driven surrogate modelling. reduced-order modelling, physic-based modelling. 

Data-driven surrogate modelling generates approximations of the high-fidelity model by using interpolation or regression of simulation data from the input/output relationships. There are popular approaches such as polynomial regression, radial basis functions, kriging, neural networks, support vector regression, Gaussian process regressions, fuzzy systems. These methods have been discussed in \cite{Forrester2009}.

\claudio{Perhaps a few words about what input output behaviour means. These can be added next to the text that introduces state space models.}
\basak{matrix form representation is necessary to clearly explain, but this is something new. So maybe we can describe it at the top ?}
\claudio{Yes good idea! We can place it after introducing State space systems (in \cref{eq:state_space}).}

Reduced-order modelling or model order reduction (MOR) are based on projection, where the high dimensional governing equations (n order) are projected onto a reduced dimension subspace characterized by a basis of orthogonal vectors. A reduced-order model represents the higher-fidelity dynamic system model by using fewer states. Mathematically, MOR can be conceived as the task of reducing the dimension of the state space from in \cref{eq:state_space_matrixform} with help of $\mathbf{z(t)} \in \mathbf{R}^{n_r}$ where $n_{r}<<n_{x}$.

\begin{equation}
    \begin{aligned}
        {x}(t) \approx Vz(t) + \in
    \end{aligned}
\end{equation}
$\text{ where } \mathbf{V} \in \mathbf{R}^{n_xXn_r} \text{ and } \in \text{ is noise}$.

The purpose of MOR is to remove the states that are uncontrollable which is the input cannot affect it and unobservable which it has no effect on the output from state-space models.

\claudio{Make link with \cref{sec:control} later.}
\begin{equation}
    \begin{aligned}
        E_{r}\dot{z}(t) = A_{r}z(t) + B_{r}u(t) \\
        y_{r}(t) = C_{r}(t)z(t) + D_{r}u(t)
    \end{aligned}
\end{equation}

The objective of the reduction is to acquire matrices $A_{r}, B_{r}, C_{r}, D_{r}, E_{r}$ in a way that $\norm{y-y_{r}}\leq AcceptedError$. At the end of reduction, the properties of the original system should be preserved, such as stability (see \cref{sec:convergence}) and passivity.

MOR can be applied manually. However, for large systems the workflow has to be automated and computationally efficient. \textbf{Krylov subspace methods} are restricted to linear systems are Krylov space methods don't rely on the singular values computation. They are known as moment-matching methods or Padé approximation methods.

Krylov space methods are applied on the problems with large sparse matrix (most element of matrix is zero) eigenvalue as a result of discretization of PDEs with the finite element method or with the finite difference method. Krylov space methods are based on iterative solution of large algebraic equations. Realization, interpolation, Lanczos, Arnoldi are algorithms used in Krylov subspaces. \textbf{SVD} (Single Value Decomposition) based MOR decompose the full-order system into a set of two orthogonal matrices and a diagonal matrix which contains the system’s singular values. This methods is divided into SVD-Based Mor for linear and nonlinear systems.

Balance Trunication and the Hankel Approximation fall under SVD-based MOR on linear systems. Balanced truncation is based upon the observation that only the largest singular values of a system are important. The Proper Orthogonal Decomposition (POD), Empirical grammians, Kernel PCA, Laplacian Eigenmaps fall under SVD-based MOR on nonlinear systems. POD method projects the original nonlinear system onto subspace with smaller dimension.

Since POD is based on the trajectory, the time response of a system (output) given a certain input contains the essential behavior of the system serves as a starting-point for POD. The datapoints are snapshots of the state space solution at different timepoints t or for different input signals. They are usually constructed by a numerical time simulation, but may also arise from measurements of a real physical system. From analysing this data, a subspace is created such that the data points as a whole are approximated by corresponding points in the subspace in a optimal least squares sense. The basis of this approach is also known as Karhunen–Loève Theorem.

Empirical grammians (empirical balanced truncation) is an extended version of a POD method due to find solutions to the issues arising in POD method. Instead of creating the reduced subspace with only one relevant input and initial state, several training trajectories are created and the reduced subspace is built. Hybrid methods try to benefit from the combination of Krylov subspace methods and SVD-based MOR for the purpose of preserve stability.

Physic-based surrogate modelling (Hierarchical surrogate models) incorporate the knowledge to form a lower-fidelity computational models by using approaches such as simplifying physical assumptions, looser residual tolerances, coarser grids. Simplified models replaces the governing equations in high-fidelity models by a set of simplified equations. Reduced numerical accuracy is where a coarser computational grid discretization is used for the same governing equations in the high-fidelity model.

\subsubsection{Design of Experiment}
\basak{DoE is a part of surrogate framework, an important part. also it is an important part of every machine learning or simulation applications. Should I keep it so we dont have to really define a section specific for this or should I remove it?}

More sample points offers more information of the function however, at higher expenses. At one point increasing sample size doesn’t contribute the accuracy of the surrogate model. Accuracy depends on weather sample points capture all the features of the function itself. Therefore, the process of data  collection for the surrogate models, which is also termed as Design  of  Experiments  (DoE) (sampling/space filling),  is  an import step on the accuracy of the surrogate model predictions.

\subsubsection{Surrogate Model Fitting}
\basak{same question here}
Model fitting is the final step of the surrogate modelling framework. The purpose of model fitting also referred as model validation, is to verify how closely the model fits the
particular training data set. Surrogate modelling framework is an iterative process between the design of experiment and model fitting until the accuracy goals are met.
\subsubsection{Surrogate Modelling and Equivalence between PCA and Auto-Encoders}
\alexandros{PCA is a linear mode, AEs in general are not. Maybe you mean that if there is an AE with one hidden layer (formed by at most D neurons, where D is the number of the input vector dimensions) using linear activation functions and imposing orthogonality constraints on the learned weights, AEs and PCA are equivalent?}
\chris{Discuss the fact that a surrogate model is a model of a model}\basak{discussed in surrogate section}
This is covered nicely in \cite{Hartman2017}.
The intuition of the Galerkin projection is better understood by understanding the link between PCA and Auto Encoders: since have that $\pi_r x_i \approx x_i$ and $\pi_r = P_r^T P_r$, then $P_r$ is mapping $x_i$ to the reduced space, and then the inverse mapping $P_r^T$ is bringing it back. To transform the derivative system we need to convert its inputs to the right space, and then convert the derivatives back to the reduced space.
Hence the result:
$$
    \dot{x}_r = P_r f ( P_r^T x_r )
$$


\subsection{Control} \label{sec:control}
\jan{The title of our paper is focusing on simulation of dynamical systems. Here I wonder whether we want to open another box with a miriad of control methods. There is so much content that it could easily take a review paper on its own. I suggest we drop control and focus only on modeling. In the literature review we can always reference model-based control papers which use neural nets for system ID. }

\chris{I agree with Jans on the point that control is big field. However, i think that work being done in control on deep koopman operators are a great example of incoporating knowledge in NNs. A solution would be introducing only the theory necessary to understand that non-linear control is difficult and that deep koopman embeddings constitute a interesting approach where a structured NN is used to solve a complex problem.}

To mention in this section:
\begin{itemize}
    \item Introduce possible controller for the pole cart system.
    \item Introduce linear quadratic regulator. (connect with stability analysis of solver. Later we can mention koopman operator for this.)
    \item State observability and controlability (reuse state space concept from previous section).
\end{itemize}

In \cref{sec:dt_models} we unceremoniously introduced an example controller for the pole-cart system.
However, one of the main reasons models are built is to help design a controller for the system those models are supposed to represent.
Once designed, the controller is deployed into the system and fine tuned to its final configuration.

For didactic purposes, we will introduce in this section the basic notions of control design for state space systems, and refer the reader to the vast literature on the topic \cite{Astrom2010,Astrom2011}.
As with other sections, the goal is to give the reader an intuition for the challenges in control design, because they too manifest themselves in DL models used for control design.

A state space system has the form of an ODE, along with equation describing how output variables are computed from state variables and inputs:
\begin{equation}\label{eq:state_space}
    \dot{x}(t) = f(x(t), u(t), \theta) \\
    y(t) = g(x(t), u(t), \theta)
\end{equation}
where $x,f,u,\theta$ are as in \cref{eq:ode}, $y(t)$ represents a vector of the measurable quantities of the system, and $g$ represent how $y$ relates to the state, inputs, and parameters.
The state space form is useful for control because it clearly separates quantities that are part of the state of the system $x$, from quantities that can be measured by sensors placed in the system.
\basak{taken from mor section, needs to be adjusted First-order coupled differential equations, together with a set of algebraic equations:}
\begin{equation}\label{eq:state_space_matrixform}
    \begin{aligned}
        E\dot{x}(t) = Ax(t) + Bu(t) \\
        y(t) = C(t)x(t) + Du(t)
    \end{aligned}
\end{equation}
where $\mathbf{x}(t) \in \mathbf{R}^{n_x}$, $\mathbf{u}(t) \in \mathbf{R}^{n_u}$, $\mathbf{y}(t) \in \mathbf{R}^{n_y}$, $\mathbf{E} \in \mathbf{R}^{n_x \times n_x}$, $\mathbf{A} \in \mathbf{R}^{n_x \times n_x}$, $\mathbf{B} \in \mathbf{R}^{n_x \times n_u}$, $\mathbf{C} \in \mathbf{R}^{n_y \times n_x}$, $\mathbf{D} \in \mathbf{R}^{n_u \times n_x}$.
\claudio{TODO: Given example of the pole cart system: what are the sensors and Internal states?}

\claudio{TODO: This section is not finished..}

\paragraph{Deep Koopman Embeddings}
A central motivation for using neural networks for modelling is that they are capable of approximating non-linear systems, which often appear in nature.
\basak{I think we should tell first what Koopman is doing and then what is the role of DL in Koopman embeddings}
Compared to linear systems, non-linear systems are much harder to identify, analyse, and control.
The idea of Koopman embeddings is to identify a mapping of the systems state-space to a latent space where the dynamics of the system become linear \cite{Lusch2018}.
$$
    \phi(x_{k+1}) = \mathcal{K} \phi(x_k)
$$
The challenge is then shifted from expressing complex non-linear dynamics to identifying a non-linear embedding $\phi$.
Identifying and representing Koopman eigenfunctions are challenging. The use of deep learning methods  {\color{red}XXX Mahdi: the last sentence is incomplete}

Recent works have attempted to parameterize the embedding using a neural network \cite{Lusch2018, Yeung2019,Boddupalli2019,Korda2018}.
\chris{finish writing}
\basak{Dont know if it is useful, just dumping some more explanation}
$x \in \mathbb{R}^{n}$, $\mathcal{K}$ is the Koopman operator.
finite dimensional but non-linear differential equations as in terms of Koopman operator which is an infinite dimensional linear operator that act on the space of all possible observable function of the state of the ordinary differential equations. Now we have linear but trade of is infinity

Continuous time differential equation like below:
$$
    \dxdt= f(x) \Rightarrow
    F_t{x(t_{0})} = x(t_{0}+t) = x(t_{0})  + \int_{\bm{t_{0}}}^{\bm{t_{0}+t}} f(x(\tau))d\tau
$$
x could be the state of a system (e.g. very high dimensional vector of fluid dynamic velocities at a bunch of point locations) If we have x at time 0, then we can integrate that initial state at some point later at time t.
This c.t.DE can be represented in discrete time update (for instance if we collect experimental data in discrete time we might need the discrete time update thinking).
$$
    x_{k+1} = F_{t}(x_{k})
$$
Koopman operator operates on the Hilbert space of observable function g on the state x. If we take Koopman operator applied to an observation at $x_{k}$, we get back measurements of the next time step.
$\circ$ means function composition
$$
    \mathcal{K}_{t}g = g \circ F_{t} \Rightarrow
    \mathcal{K}_{t}g(x_{k}) = g(F_{t}(x_{k})) =  g(x_{k})
$$
Continuous version would be :
$$
    \frac{d}{dt} g= \mathcal{K}g \\
$$
The linear infinite dimensional $\mathcal{K}$ tells us what the measurements will be in the next time step. But these observable functions live in an infinite dimensional Hilbert space so $\mathcal{K}$ might be really complicated. Therefore, for instance \cite{Lusch2018} is using deep learning to find the eigenfunction of Koopman.

\subsection{State Estimation}
\chris{This section should discuss the issue of starting a simulation when the initial state is unknown or only partially obeseved.}

\subsubsection{Estimating Initial State}
For some applications the initial state, $x_0$, is unknown, or we may only have estimates a of subset of state variables.
\chris{Describe the different approaches we have observed for estimating initial state from either partial or corrupt state estimates. This is tightly linked to taking multiple states as input. For example consider case of a pendulum where the initial state is partial and only includes the position of the pendulum. In this case a single sample is not sufficient to determine if the pendulum is swinging left or right. Likewise relying on a single noisy sample of the initial state will result in a large simulation error}

\paragraph{Hidden Physics Networks}
Related to using neural networks as simulators is using them to enrich the results of already-executed simulations, by having them estimate physical quantities not present in the original simulation by enforcing physical constraints.
This has been applied to extract velocity and pressure fields using only the concentration of a dye as input \cite{Raissi2020}.

\chris{cover this as well \cite{Raissi2018}}


==> sections/old_5_discussion.tex <==
\section{Research Gaps and Directions}
\label{sec:discussion}

The previous sections outlined the basic concepts necessary to construct models of dynamical systems using NNs.
One take-away from this is that there are multiple ways of constructing a model capable of producing prediction of a system's trajectory.
Specifically, we saw that an ideal pendulum could be modeled accurately using both direct-solution and time-stepper models and that several variants of each model can be applied.

A natural question to ask is whether these techniques work well in practice when dealing with more complicated real-life systems (\cref{sec:disc_benchmarks}).
Another is how much data is required to provide a sufficiently accurate model of a system and finding robust procedures for training (\cref{sec:discussion_training_ts}).
Unlike the ideal pendulum, the ODEs or PDEs governing a physical system are generally not known; which is the key motivation for using data-driven modeling in the first place.
Measuring large quantities of data from a physical system is significantly more difficult than obtaining it by simulating a set of differential equations.

Another issue of NN-based models is that they are difficult to analyze compared to hand-crafted models (\cref{sec:disc_reliability}).
Consequently, this makes it hard to provide formal guarantees that the error of the prediction will stay within a certain limit.
This issue can be seen in relation to the fact that NNs are generic structures that can be applied to many types of problems.
It seems almost paradoxical that we are using a black-box model to solve a problem --- while expecting the results to be interpretable.
Despite this, we have already seen several ways that the network can be used in a way that allows its output to be reinterpreted in a meaningful way.
For instance, the network inside a time-stepper model is used to estimate the derivative, which is then used by a traditional solver to predict the state one step into the future.
Using this interpretation allows us to use a network to model the system's dynamics, while at the same leveraging the knowledge from numerical simulation.
Related to this is the need for visualization techniques which may aid in understanding the dynamics acquired by the trained model (\cref{sec:desc_visualization}).

\subsection{Lack of benchmarks for comparison}
\label{sec:disc_benchmarks}

A crucial factor that has contributed to the sustained growth of deep learning applications is the availability of large, high quality, benchmark datasets~\cite[19]{Goodfellow2016}.
The popularity of these benchmark has enabled researchers to compare results on equal footing, thereby allowing them to quickly evaluate the effectiveness of proposed methods.

Unfortunately, unlike image processing related tasks, the use of NNs for simulating dynamical systems have not yet received the same kind of attention. 
At the time of writing, the majority of papers are applied to simple, idealized examples of physical systems such as an ideal-pendulum, or directly to mathematical equations such as a wave function.
At these hand-picked problems, each paper demonstrates high performance. 
However, the fact that they are applied to different problems with varying complexity makes it difficult to determine which of the proposed methods is worthwhile pursuing.

A pressing need is to collect large amounts of data from different types of dynamical systems and compile this into a benchmark for training ML models.
In order to study the effectiveness of the methods, the systems from which the data is collected should be diverse and range in complexity.
For example, the benchmark could include variations of a problem such as a pendulum. 
In the simplest case the system may be an ideal-pendulum, slightly more advanced a 2-link pendulum, and finally data from physical pendulum, influenced by non-linear friction terms, elasticity, etc.
Additionally, the benchmark could contain examples of systems that are representative of the challenges that must be dealt with during modeling such as: measurement noise, partially observed state, external inputs, time-varying dynamics.

Only once this preliminary work is completed, the research can move from being proof of concept towards demonstrating the feasibility of real world applications.

Creating high quality datasets is a huge undertaking, especially in the case where data must be captured from a physical system. Rather than creating it from scratch, it may advantageous to collect existing datasets from intersecting disciplines such as system identification and control.
For instance, there has already been efforts into collecting and curating datasets for system identification \cite{Moor1997,Schoukens2017,Kroll2014}.
Collecting multiple datasets, representative of a wide range of domains, into a single benchmark have be a benefit for the community.
This would allow us to study fundamental questions like determining which types of models work well across multiple problems and what the best procedure is for training such models.

\subsection{Training of Time-Steppers Models} \label{sec:discussion_training_ts}

The goal of training a time-stepper model is to obtain a model which can accurately predict the trajectory of the system several steps into the future starting from a given initial condition.
A useful property of traditional numerical solvers is that they allow the user to define the step-size used by the solver, allowing the user to control the numerical error caused by discretization as well as defining the timespan of a simulation.
Likewise, a desirable property of a trained time-stepper model is that it will work with different step-sizes after training.
However, this is rarely the case, if certain steps, described below, are not taken.

It is possible to train a time-stepper on data corresponding to a certain step-size and obtain great performance, only to have the performance deteriorate when performing predictions of a different step size.
This can be demonstrated empirically by plotting the derivatives produced by two identical Euler time-stepper, trained to minimize the single-step error, as shown in \cref{fig:ts_phase_portrait_train_stepsize_small} and \cref{fig:ts_phase_portrait_train_stepsize_large}.
It can be seen that training on data corresponding to a smaller step-size results in a phase portrait which is relatively close to the ODE used to generate the data.
Conversely, the phase portrait of the model trained with a large step-size results display drastically different dynamics.
Note that this happens, even when a very small single-step error has been achieved for both models.
\begin{figure}
    \centering
    \begin{subfigure}{0.40\textwidth}
		\centering
		\includegraphics[width=\textwidth]{figures/discussion/phase_portrait_train_stepsize_0.010.pdf}
		\caption{Small step of 0.01 seconds. The phase portrait shows that the derivatives produces by the network are close to those of the true system.}
		\label{fig:ts_phase_portrait_train_stepsize_small}
    \end{subfigure}
    \hspace{1cm}
    \begin{subfigure}{0.40\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/discussion/phase_portrait_train_stepsize_1.000.pdf}
        \caption{Large step of 1.0 seconds. The phase portrait shows that the derivatives produced by the network result in a single point of attraction in (0,0), which does not match the true system.}
        \label{fig:ts_phase_portrait_train_stepsize_large}
    \end{subfigure}
    \caption{Influence of step size used during training on the dynamics acquired by the model.}
    \label{fig:ts_training_convergence}
\end{figure}
An intuitive explanation of this phenomenon is that there is an interplay between the derivative produced by the NN and the integration step which depends on the step-size.
Specifically, it is possible for the NN to produce incorrect derivatives which, when paired with a specific integration scheme and step-size, just so happens to provide a fit in the training points.
This is illustrated in \cref{fig:ts_step_size_derivative_interplay}, which shows how taking one big step, using an incorrect derivative may reach the same state as taking several smaller steps while using the correct derivative.
This single step \emph{shortcut} is tied to the step size, and when taken with a different step size, causes the prediction to deteriorate, as shown in green in the figure.
\begin{wrapfigure}{R}{0.60\textwidth}
        \centering
        \includegraphics[width=0.55\textwidth]{figures/discussion/step_size_derivative_interplay.pdf}
        \caption{Interplay between step-size used during training and the step-size used during evaluation. If the network is trained to minimize the error one step into the future, it is prone to learn incorrect derivatives if a large step size is used.}
        \label{fig:ts_step_size_derivative_interplay}
\end{wrapfigure}
For a system such as the ideal pendulum, where the derivatives are well known, it is straightforward to examine the step-size used during training effects the learned dynamics.
However, consider the case of modeling a physical system where the dynamics are unknown and only data corresponding to a specific sampling rate is available.
Seen in the context of the ideal pendulum, if given a sparse sampling of the signal corresponding to $h = 1.0$ seconds, it would be easy to make the mistake and conclude that the model producing the phase portraits shown in \cref{fig:ts_phase_portrait_train_stepsize_large}, is a good approximation of the true system.

There are potentially many factors influencing this phenomenon.
An important one of these is how the time-stepper is trained.
Empirically, we demonstrated that minimizing the single-step loss using training data corresponding to a large step-size may manifest itself as incorrect gradients.
An alternative approach to training, would be forcing the network to take several shorter steps in between two points in the training data, rather than just a single step.
Forcing the network to take multiple steps would conceivably eliminate the particular scenario depicted in \cref{fig:ts_step_size_derivative_interplay}.

The proposed approach of taking multiple steps can be viewed as a \emph{collocation method}, in the sense that we are searching for a set of parameters that results in a trajectory passing through a set of collocation points.
Specifically, for training a time-stepper model, the parameters are the coefficients of the network that implement the dynamics of the system.
Other related methods come from \emph{trajectory optimization}, which seeks to solve a very similar problem \cite{Betts1998}.
In this type of problem, where the dynamics of the system are known, and the challenge lies in determining how to get the system from point A to point B in an optimal way.

\subsection{Reliability and Validation} 
\label{sec:disc_reliability}

An inherent challenge of data-driven modeling is evaluating how well the trained model works data representative for the real life application of the model.
A common approach is to evaluate the performance of the model on a partition of data that has not been used during training.
The underlying assumption is that this will give an unbiased estimate of how well the model works with the data that will be encountered in the final application.
The concrete validation procedure depends on which type of model that has been constructed.

Consider a direct-solution model that has been trained to produce a simulation corresponding to a specific initial condition.
In this case it does not make sense to examine the ability to generalize to different initial conditions, since there is no way to do this without retraining the model.
Instead, the models ability to produce accurate predictions corresponding to time instances that have not been used during training.
A plot like the one shown in \cref{fig:prediction_continuous_model_vanilla} can be used to visualize how well the predictions fit the underlying system.
A challenge of doing this for real life applications is that we might not have enough samples of the true system to form a dense trajectory like that shown in \cref{fig:prediction_continuous_model_vanilla}.
Without this validation procedure, it would be tempting to conclude that any of the continuous time models provided an equally good fit to the underlying dynamics.
 
Alternatively, known invariants of a particular system (such as energy conservation, recall \cref{sec:ts_energy_based}) can be leveraged by plotting the total energy of the system at every time-step.
This would allow verification despite not having access to a densely sampled trajectory of the system.

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=.65\columnwidth]{figures/discussion/ideal_pendulum_TimeStepperEuler_101_steps.pdf}
%     \caption{Error per initial condition for Euler time-stepper, each simulated for 100 steps.}
%     \label{fig:pendulum_error_heatmap}
% \end{figure}

For time-stepper models, where it should be possible to simulate for different initial conditions, the validation process should reflect this by examining how well the model works for different initial conditions.
For the examples of time-steppers models shown in this paper we have trained and validated the result in the following way: (1) the network is trained on 100 trajectories of a single step starting from initial conditions sampled using latin hyper-cube sampling as seen in \cref{fig:ts_training_data}, (2) the network is validated by sampling initial conditions in a grid and simulating 100 steps forward in time as shown in \cref{fig:true_vs_predicted_euler}.
Starting the simulation of the validation trajectories from an initial condition not encountered during training limits any effect of overfitting.

% Another way of visualizing the error associated with simulating from a specific initial condition is to use a heatmap like the one shown in \cref{fig:pendulum_error_heatmap}.
% From the plot it appears that the error is generally low, except for some corners where the error appears to be significantly higher.
% At a practical level, the plot is produced by computing the error between the trajectories of the true system and the model for several initial conditions and assigning each point a color representative of the error.
% Sampling the initial conditions used for validation in a grid is useful as it simplifies the interpolation process that gives the impression of a continuous heatmap.
% \claudio{Consider maybe moving some details above into the caption of \cref{fig:pendulum_error_heatmap} as maybe it is easier for the reader to read them while looking at the figure.}
% An obvious limitation of this approach is that it requires a significant number of trajectories to create a sufficiently dense heatmap and that the technique cannot be applied to high dimensional systems.

An important piece of future work is to develop a set of techniques and best practices for validating data-driven models of dynamical systems.
Simulation is a unique problem compared to other application such as classification or forecasting a single step into the future.
These techniques should utilize the existing knowledge of dynamical systems to provide a measure of the trained models predictive capabilities.

This problem has parallels with the traditional challenge of understanding the limits of handcrafted models and the experimental context in which they are obtained (see, e.g., \cite{Denil2017} for an introduction), and can be tackled in practice with a combination of documentation, traceability, reproducibility packages, as well as improved visualization, as proposed next.

\subsection{Visualization of High Dimensional Dynamics}
\label{sec:desc_visualization}

So far, we have considered cases where a network is trained successfully --- allowing the model to produce accurate predictions for all possible initial conditions.
However, prior to reaching this point is an iterative process of tweaking the structure and experimental setup used during training and validation of the model.
The ability to reason about the causes of the poor performance is the difference between optimizing the structure blindly or in a structured way that is likely to converge on good results.

An important tool to develop understanding is visualization.
A concrete example of this is the phase portrait shown in \cref{fig:pendulum_phase_portrait}.
By looking at this figure, we can instantly get an impression of how trajectories will evolve for any initial condition in the state-space.

Unfortunately, these techniques are only possible to apply directly for systems where the state-space is at most 3 dimensional.
A classical solution to this is to combine the information from several states into a smaller number of states that can then be rendered.
There are many possible ways to encode information such as using color or symbol shapes~\cite{Wegenkittl1997}.
Another approach is to determine a mapping from the high-dimensional state-space to a lower dimensional space that can readily be plotted using techniques such phase portraits.
The usefulness of a mapping relies on two factors: (a) the ease of which a human can interpret the data, (b) that the mapping preserves relevant characteristics of the high-dimensional data.
For example, when embedding several high-dimensional trajectory in a low-dimensional space we would like similar trajectories to remain similar and vice versa.
The authors of~\cite{Bartolovic2020} propose a technique that preserves characteristics asymptotic convergence and continuity of the projected trajectories.

A different approach is to create a virtual model of the system and represent each state variable by their physical significance.
For instance, the angle and angular velocity of a pendulum can be represented by rotating the geometry of a 2-D model.
To compare the predicted and true trajectories, two virtual models can be shown side by side or overlapping, with one of the virtual models being made translucent.
This type of visualization is often encountered in the context of \emph{reinforcement learning}~(RL).
A subdomain of reinforcement learning is obtaining continuous control algorithms for complex non-linear systems \cite{Duan2016}. 

==> tables/table_knowledge.tex <==
\begin{tabular}{lllll}
\toprule
{} & Structure & Loss & Feature Engineering & Hybrid Model \\
\midrule
Doe2020  &         \checkmark &    \checkmark &                   \checkmark &            \checkmark \\
Bong2010 &         \checkmark &    \checkmark &                     &              \\
Jane2019 &         \checkmark &      &                     &            \checkmark \\
\bottomrule
\end{tabular}


==> tables/table_model.tex <==
\begin{tabular}{lllllll}
\toprule
{} & Estimation & Step & External-Input & Partial State & Past Input & Noise \\
\midrule
Doe2020  &          D &    F &              \checkmark &               &            &       \\
Bong2010 &          D &    A &                &               &            &       \\
Jane2019 &          G &    F &                &               &          \checkmark &     \checkmark \\
\bottomrule
\end{tabular}


==> tables/table_objective.tex <==
\begin{tabular}{llll}
\toprule
{} & Purpose & Industry Domain & Physical Phenomena \\
\midrule
Doe2020  &       H &            HVAC &     Thermodynamics \\
Bong2010 &       D &      Automotive &         Hydraulics \\
Jane2019 &       G &         Science &            Quantum \\
\bottomrule
\end{tabular}


==> tables/table_quality.tex <==
\begin{tabular}{lll}
\toprule
{} & Validation & Source \\
\midrule
Doe2020  &        TTV &     UE \\
Bong2010 &         TV &     CE \\
\bottomrule
\end{tabular}

